Fast Graphlet Transform of Sparse Graphs

We introduce the computational problem of graphlet transform of a sparse large graph. Graphlets are fundamental topology elements of all graphs/networks. They can be used as coding elements to encode graph-topological information at multiple granularity levels for classifying vertices on the same graph/network as well as for making differentiation or connection across different networks. Network/graph analysis using graphlets has growing applications. We recognize the universality and increased encoding capacity in using multiple graphlets, we address the arising computational complexity issues, and we present a fast method for exact graphlet transform. The fast graphlet transform establishes a few remarkable records at once in high computational efficiency, low memory consumption, and ready translation to high-performance program and implementation. It is intended to enable and advance network/graph analysis with graphlets, and to introduce the relatively new analysis apparatus to graph theory, high-performance graph computation, and broader applications.

==> Makefile <==
############################################################
#	 	    LaTeX makefile
#

### SHELL SYNTAX

SHELL := /bin/bash

### COMMANDS

LATEX   = pdflatex --synctex=1 -file-line-error
BIBTEX  = bibtex
RM      = rm -rf

### TARGETS

T_DOC = fast-graphlets-main


### CLEAN-UP EXTENSIONS

EXT_CLEAN = .tex~ .pdfsync \
	    .out \
	    .dvi \
	    .pdf \
	    .aux \
	    .toc \
	    .lof \
	    .lot \
	    .log \
	    .blg \
	    .brf \
	    .nav \
	    .snm \
            .spl \
	    .glg \
	    .glo \
	    .gls \
	    .ist \
	    .idx \
	    .ilg \
            .fls \
            .fdb_latexmk \
	    .synctex.gz \
	    .run.xml \
	    -blx.bib \


### COMPILATION / MAKE

# PHONY targets are always compiled
.PHONY: all clean

# default "make" target
.DEFAULT_GOAL := all

# "regular"
all: clean			## HPEC mode
	$(LATEX)  "\input{$(T_DOC)}"
	$(BIBTEX) $(T_DOC)
	$(LATEX)  "\input{$(T_DOC)}"
	$(LATEX)  "\input{$(T_DOC)}"


clean:				## Clean LaTeX files (incl. PDF)
	$(RM) $(addprefix $(T_DOC),$(EXT_CLEAN))
	$(RM) texput.log


